Separation and Encodability in Mixed Choice Multiparty Sessions (Technical Report)

Multiparty session types (MP) are a type discipline for enforcing the structured, deadlock-free communication of concurrent and message-passing programs. Traditional MP have a limited form of choice in which alternative communication possibilities are offered by a single participant and selected by another. Mixed choice multiparty session types (MCMP) extend the choice construct to include both selections and offers in the same choice. This paper first proposes a general typing system for a mixed choice synchronous multiparty session calculus, and prove type soundness, communication safety, and deadlock-freedom. Next we compare expressiveness of nine subcalcli of MCMP-calculus by examining their encodability (there exists a good encoding from one to another) and separation (there exists no good encoding from one calculus to another). We prove 8 new encodablity results and 20 new separation results. In summary, MCMP is strictly more expressive than classical multiparty sessions (MP) and mixed choice in mixed sessions. This contrasts earlier results where mixed sessions do not add any expressiveness to non-mixed fundamental sessions, shedding a light on expressiveness of multiparty mixed choice.

==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

We introduced a variant of multiparty session types with mixed choice and proved the introduced variant of mixed choice in terms of expressiveness is comparable to mixed choice in the $ \pi $-calculus.
We studied several subcalculi to analyse what exactly causes an increase in the expressive power of the considered choice constructs.
As already with the $ \pi $-calculus an increase results from separate and mixed choice but only if we all to combine different communication partners in a choice.

To simplify the calculus and not clutter our analysis, \mcmpst and all its variants describe a single session without shared names or delegation.
We leave the study of interleaved sessions, delegation, shared channels, and the session invitation mechanism for further research.
Indeed the typical synchronous session initialisation on shared names for multiparty sessions, where a session request $ \overline{a}[n](s).P $ is matched with several session acceptances $ a[i](s).Q_i $ in a rule such as
\begin{align*}
	&\overline{a}[n](s).P \Par a[1](s).Q_1 \Par \ldots \Par a[n-1](s).Q_n\\
	&\red (\nu s) \left( P\subst{s[n]}{s} \Par Q_1\subst{s[1]}{s} \Par \ldots \Par Q_n\subst{s[n-1]}{s} \right)
\end{align*}
is very expressive.
Calculi with this or a similar session initialisation can express \eg the \patternStar without any choice.
Also note, that the \patternM that we find in \cnv and \cnvms are caused by unrestricted channels and not choice as we can clearly see in $ \PM_{\cnv} $ in the sixth row and $ \PM_{\text{\cnvms}} $ in the seventh row of Figure~\ref{fig:KeysExpressiveness}.
Accordingly, we first studied calculi without shared names or session initialisation.

Another interesting topic for further research is a comparison of \scmpst with the $ \pi $-calculus with separate choice and of \mcmpst with the $ \pi $-calculus with mixed choice.
As discussed the introduced variants of separate choice in \scmpst and mixed choice in \mcmpst are comparable with the respective variants of choice in the $ \pi $-calculus.
This observation is also supported by the study of the more practical problem of leader election in symmetric networks.
The exact relationship between \scmpst and the $ \pi $-calculus with separate choice and between \mcmpst and the $ \pi $-calculus with mixed choice is, however, still open.
Remember that \scmpst and \mcmpst are typed calculi that ensure \eg deadlock-freedom but the $ \pi $-calculus does not.
An interesting question is for instance how much deadlock-free processes cannot be well-typed in \mcmpst.

==> diagram.tex <==
\begin{figure*}
\begin{tabularx}{\textwidth}{m{5.6cm}c}
	\footnotesize
	\begin{tikzpicture}[x=10mm, y=21mm, scale=0.25]
		\tikzstyle{setNumber}=[circle, inner sep = 2, draw, fill=white]
		\tikzstyle{common-attributes} = [rounded corners, ultra thick]

		% local contexts
		\draw[common-attributes]	(0, 0) rectangle (22.5, 11);
		\node[setNumber]		at	(2, 2)		{\tiny 1};
		
		% safe
		\draw[common-attributes, draw=cyan!80]
									(3, 0.5) rectangle (20.5, 10.5);

		\node[setNumber, left]	at	(11.75, 1)		{\tiny 2};
		\node[right]			at	(11.75, 1)		{\footnotesize \color{cyan!80} \safe{\LL}};

		% deadlock-free - sets 3 and 5
		\draw[common-attributes, draw=magenta]
									(1, 3) rectangle (21.5, 10);

		\node[setNumber]		at	(2, 7.5)		{\tiny 3};
		\node[setNumber, left]	at	(11.25, 9.5)	{\tiny 5};
		\node[right]			at	(11.25, 9.5)	{\footnotesize \color{magenta} \df{\LL}};

		% projected - sets 4 and 7
		\draw[common-attributes, draw=orange]
									(4, 1.5) rectangle (19.5, 7.5);

		\node[setNumber, left]	at	(11.75, 2.25)	{\tiny 4};
		\node[right]			at	(11.75, 2.25)	{\footnotesize \color{orange} $\projset{\glob}$};
		\node[setNumber, left]	at	(11.75, 3.75)	{\tiny 7};
		\node[right]			at	(11.75, 3.75)	{\footnotesize \color{magenta} $\df{\color{orange} \projset{\glob}}$};

		% live - sets 6 and 8
		\draw[common-attributes, draw=olive]
									(5, 4.5) rectangle (18.5, 9);
		\node[setNumber, left]	at	(11.75, 8.25)		{\tiny 6};
		\node[right]			at	(11.75, 8.25)		{\footnotesize \color{olive} $\live{\LL}$};
		
		\node[setNumber, above]	at	(8.5, 5.5)		{\tiny 8};
		\node[below]			at	(8.5, 5.5) 		{\footnotesize {\color{olive} $\live{\color{orange} \projset{\glob}}$}};


		% well-behaved projection
		\draw[common-attributes, draw=violet]
										(10.5, 5.5) rectangle (17.5, 7);
		\node[setNumber, above]		at	(14, 6.25) {\tiny 9};
		\node[below]				at	(14, 6.25) {\color{violet}  $\glob \wb \projset{\glob}$};

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\end{tikzpicture}
		 &
		$
			\footnotesize
			\begin{array}{c|r@{\ }l|c}
				\hline
				\hline

				\parbox[h][.54cm]{0cm}{}
				\tikz[baseline=(i.base)]{\node[circle, draw, fill=white, inner sep = 2] (i){\scriptsize $i$};}
				& \multicolumn{2}{c|}{\text{Local
                                    Context Example}}
				                                 & \text{Properties}
				\\[1mm]
				\hline
				1
				                                 & \LLi{1}	=                                                                             
												 & \p: \ntoutlbl{\q}{\lab}{\nat}, \q: \ntinplbl{\p}{\lab}{\bool}
				                                 & \neg\safe{\LLi{1}}, \neg\df{\LLi{1}}
				\\[1mm]
				\hline
				2
				                                 & \LLi{2} =                                                                            
												 & \p: \ntout{\q}{\lab}
				                                 & \safe{\LLi{2}},\ \neg\df{\LLi{2}}
				\\[1mm]
				\hline
				3
				                                 & \LLi{3}	=                                                                             
												 & \p: \trec{t}{\tout{\q}{\lab_1} \tvar{t}}, \rr: \ntoutlbl{\roled{r}}{\lab_2}{\nat},
				                                 & \df{\LLi{3}},\ \neg\safe{\LLi{3}}
				\\
				                                 && \q: \trec{t}{\tinp{\p}{\lab_1} \tvar{t}}, \roled{r}: \ntinplbl{\rr}{\lab_2}{\bool} &                                                                                                            
				\\[1mm]
				\hline
				4
				                                 & \LLi{4} =                                                                            
												 & \projset{\globnodf}
				                                 & \neg\df{\projset{\globnodf}}
				\\[1mm]
				\hline
				5
					& \LLi{5} =
					& \p: \trec{t}{\tout{\q}{\lab_1} \tvar{t}}, \rr: \ntoutlbl{\roled{r}}{\lab_2}{\nat},
					& \df{\LLi{5}},\ \safe{\LLi{5}}
				\\ && \q: \trec{t}{\tinp{\p}{\lab_1} \tvar{t}}& \neg\live{\LLi{5}}
				\\[1mm]
				\hline
				6
					& \LLi{6}	= 
					& \p: \ntout{\q}{\lab_1} \tor \ntout{\q}{\lab_2}, \q: \ntinp{\p}{\lab_1}
					& \live{\LLi{6}}
				\\		&&& \not\exists, \glob, \LLi{6} = \projset{\glob}
				\\[1mm]
				\hline
				7
					& \LLi{7} =
					& \projset{\globnolive} %\LLi{4}, \rr: \trec{t} \tout{\roled{r}}{\lab} \tvar{t},
					& \df{\LLi{7}}, \neg\live{\LLi{7}}
				\\[1mm]
				\hline
				8
					& \LLi{8} =
					& \projset{\globringone}
					& \globringone \not\wb \LLi{8}
				\\[1mm]
				\hline
				9
					& \LLi{9} =
					& \projset{\globringtwo}
					& \globringtwo \wb \LLi{9}
				\\
				\hline
				\hline
			\end{array}
		$
	\end{tabularx}
	%\Description{A diagram}

	% \caption{The set relationship between safety, deadlock-freedom,
	% 	liveness and projection in local contexts
	% 	\label{fig:properties}. $\LLi{i}$ in ``Type''
	% 	represents an example which belongs to
	% 	the corresponding set $i$ in the venn diagram. ``Properties'' mean
	% 	the property (un)satisfied $\LLi{i}$.}

	\caption{The relationship between deadlock-freedom, live,
		projectability, and conformance properties on local contexts
		\LL and global types \glob (Left); and
		an example of local contexts for each region (Right).
                For the $i^{th}$ region we provide a local context and 
		explicitly specify which properties it does/does not
                satisfy. For example,  the $5^{th}$ region (left)  
                denotes local contexts which are safe and deadlock-free, but not
                live, and $\LLi{5}$ in the table (right) is an
                example which is safe and deadlock-free, but not live. }
\vspace*{-3mm}
		\label{fig:properties}
\end{figure*}


==> figures/fig-hierarchy-full.tex <==
{\scriptsize
\begin{figure*}
	\renewcommand{\arraystretch}{1.2}
	\arraycolsep2pt
	\begin{tabular}{|l|l|c|}
		\hline
		1 &
		$ \begin{array}{l}
			\scbs \blueArrow \bs\\
			\smpst \blueArrow \mpst
		\end{array} $ &
		$ \begin{array}{rcl}
			\ArbitraryEncoding{\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I}} &=& \choice{\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I}\\
			\ArbitraryEncoding{\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J}} &=& \colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J}
		\end{array} $\\
		\hline
		2 &
		$ \begin{array}{l}
			\mcbs \blueArrow \scbs\\
			\dmpst \blueArrow \smpst
		\end{array} $ &
		$ \begin{array}{l}
			\ArbitraryEncoding{\left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I} \right) \OR \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J} \right)}\\
			= \begin{cases}
				\begin{array}{l}
					\left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right) \OR\\
					\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\left( \left(\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{yellow!30}{\ssinp{\q}{\lbl{reset}}}\seq \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right)
				\end{array} & \text{if } I \neq \emptyset \neq J \wedge \p < \q\\
				\left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } I \neq \emptyset \neq J \wedge \p > \q\\
				\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p < \q\\
				\colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p > \q\\
				\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} & \text{if } I = \emptyset \wedge \p < \q\\
				\left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\colorbox{yellow!30}{\ssout{\q}{\lbl{reset}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} & \text{if } I = \emptyset \wedge \p > \q
			\end{cases}
		\end{array} $\\
		\hline
		3 &
		$ \begin{array}{l}
			\mcbs \blueArrow \bs\\
			\dmpst \blueArrow \mpst
		\end{array} $ &
		$ \begin{array}{l}
			\ArbitraryEncoding{\left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I} \right) \OR \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J} \right)}\\
			= \begin{cases}
				\begin{array}{l}
					\left( \choice{\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right) \OR\\
					\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\left( \left(\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{yellow!30}{\ssinp{\q}{\lbl{reset}}}\seq \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right)
				\end{array} & \text{if } I \neq \emptyset \neq J \wedge \p < \q\\
				\colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\left( \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right) & \text{if } I \neq \emptyset \neq J \wedge \p > \q\\
				\choice{\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p < \q\\
				\colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p > \q\\
				\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} & \text{if } I = \emptyset \wedge \p < \q\\
				\colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\left( \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\colorbox{yellow!30}{\ssout{\q}{\lbl{reset}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) & \text{if } I = \emptyset \wedge \p > \q
			\end{cases}
		\end{array} $\\
		\hline
		\multirow{2}{*}{4} &
		\multirow{2}{*}{\mpst \redArrow \mcbs} &
		three distributable steps in\\
		&& $ M_{\mpst} = \pa{\role{a}}{\left( \ssout{\role{b}}{l}\seq\success \OR \ssout{\role{b}}{l}\seq\inact \right)} \Par \pa{\role{b}}{\ssinp{\role{a}}{l}\seq\inact} \Par \pa{\role{c}}{\left( \ssout{\role{d}}{l}\seq\success \OR \ssout{\role{d}}{l}\seq\inact \right)} \Par \pa{\role{d}}{\ssinp{\role{c}}{l}\seq\inact} \Par \pa{\role{e}}{\left( \ssout{\role{f}}{l}\seq\success \OR \ssout{\role{f}}{l}\seq\inact \right)} \Par \pa{\role{f}}{\ssinp{\role{e}}{l}\seq\inact} $\\
		\hline
		\multirow{2}{*}{5} &
		\scmpst \redArrow &
		the synchronisation pattern \patternM in\\
		& Bottom Layer &
		$ \PM_{\scmpst} = \pa{\enodei{a}} \left( \ssout{\enodei{b}}{l}. \ssout{\enodei{d}}{l}. \inact \OR \ssout{\enodei{d}}{l'}. \inact \right) \Par \pa{\enodei{b}} \left( \ssinp{\enodei{a}}{l}. \inact \OR \ssinp{\enodei{c}}{l}. \inact \right) \Par \pa{\enodei{c}} \left( \ssout{\enodei{b}}{l}. \inact \OR \ssout{\enodei{d}}{l}. \inact \right) \Par \pa{\enodei{d}} \left( \ssinp{\enodei{c}}{l}. \ssinp{\enodei{a}}{l}. \success \OR \ssinp{\enodei{a}}{l'}. \inact \right) $\\
		\hline
		\multirow{2}{*}{6} &
		\cnv \redArrow &
		the synchronisation pattern \patternM in\\
		& Bottom Layer &
		$ \PM_{\cnv} = \ResCMV{x}{y}{\left( \OutCMV{x}{\true}{\inactCMV} \Par \InpCMV{\linCMV}{y}{z}{\ConditionalCMV{z}{\inact}{\inactCMV}} \Par \OutCMV{x}{\false}{\inactCMV} \Par \InpCMV{\linCMV}{y}{z}{\ConditionalCMV{z}{\inactCMV}{\success}} \right)} $\\
		\hline
		\multirow{2}{*}{7} &
		\cnvms \redArrow &
		the synchronisation pattern \patternM in\\
		& Bottom Layer &
		$ \PM_{\text{\cnvms}} = \ResCMVmix{x}{y}{\left( \ChoiceCMVmix{\linCMV}{x}{\OutCMVmix{l}{\true}{\inactCMVmix}} \Par \ChoiceCMVmix{\linCMV}{y}{\InpCMVmix{l}{z}{\ConditionalCMVmix{z}{\inact}{\inactCMVmix}}} \Par \ChoiceCMVmix{\linCMV}{x}{\OutCMVmix{l}{\false}{\inactCMVmix}} \Par \ChoiceCMVmix{\linCMV}{y}{\InpCMVmix{l}{z}{\ConditionalCMVmix{z}{\inactCMVmix}{\success}}} \right)} $\\
		\hline
		\multirow{4}{*}{8} &
		& the synchronisation pattern \patternStar in\\
		& \msmpst \redArrow &
		$ \PS_{\msmpst} = M_{\enodei{a}} \Par M_{\enodei{b}} \Par M_{\enodei{c}} \Par M_{\enodei{d}} \Par M_{\enodei{e}} \Par M_{\enodei{gc}} \hspace{2em} M_{\enodei{a}} = \pa{\enodei{a}} \left( \ssout{\enodei{e}}{l}. \inact \OR \ssinp{\enodei{b}}{l}. P_{\enodei{a}} \OR \ssinp{\enodei{gc}}{\delete}. \inact \right) $\\
		& Lower Layers &
		$ M_{\enodei{gc}} = \choice{\ssout{\enodei{i}}{\delete} \seq \inact}{\enodei{i} \in \set{\enodei{a}, \enodei{b}, \enodei{c}, \enodei{d},\enodei{e}}} \hspace{2em} \sigma = \left[ \enodei{a} \mapsto \enodei{b}, \enodei{b} \mapsto \enodei{c}, \enodei{c} \mapsto \enodei{d}, \enodei{d} \mapsto \enodei{e}, \enodei{e} \mapsto \enodei{a} \right] $\\
		&& $ M_{\enodei{b}} = M_{\enodei{a}}\sigma \quad M_{\enodei{c}} = M_{\enodei{b}}\sigma \quad M_{\enodei{d}} = M_{\enodei{c}}\sigma \quad M_{\enodei{e}} = M_{\enodei{d}}\sigma \hspace{2em} P_{\enodei{a}}, \ldots, P_{\enodei{e}} \in \left\{ \success, \inact \right\} $\\[1mm]
		\hline
		9 &
		\mcmpst \blueArrow \msmpst &
		$ \begin{array}{l}
\ArbitraryEncoding{\sum_{\q} \left( \left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I} \right) \OR \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J} \right) \right)} %\\
			= \sum_{\q}
			\begin{cases}
				\text{case distinction of \mcbs \blueArrow \scbs}
			\end{cases}
		\end{array} $\\[1mm]
		\hline
		10 &
		\mcbs \redArrow \lcnvms &
		$ M_{\mcbs} = \pa{\p}{\left( \ssout{\q}{l_1}\seq\inact \OR \colorbox{orange!20}{\ensuremath{\ssinp{\q}{l_2}\seq\success}} \right)} \Par \pa{\q}{\left( \ssinp{\p}{l_1}\seq\inact \OR \colorbox{orange!20}{\ensuremath{\ssinp{\p}{l_3}\seq\success}} \right)} $\\
		\hline
		11 &
		\lcnvms \blueArrow \mcbs &
		$ \begin{array}{l}
\, 			\ArbitraryEncoding{\Gamma \vdash \ResCMVmix{x}{y}{\PP}} = \ArbitraryEncoding{\Gamma' \vdash \PP}_{x, y}\\
			\ArbitraryEncoding{\Gamma \vdash \ChoiceCMVmix{\linCMVmix}{\mathsf{k}}{\left( \PP = \left( \sum_{i \in I} \OutCMVmix{\lab_i}{v_i}{\PP_i} \right) \OR \left( \sum_{j \in J} \InpCMVmix{\lab_j}{z_j}{\PP_j} \right) \right)}}_{x, y}\\
			= \begin{cases}
				\pa{\enodei{k}}{\inact} & \text{if } \fv{\PP} = \Set{x, y} \cup \Set{\mathsf{k}}\\\
				\pa{\enodei{k}}{\left( \sum_{i \in I} \soutprlbl{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{o}}{v_i}\seq\ArbitraryEncoding{\Gamma_i \vdash \PP_i}_{\mathsf{\overline{k}}} \right)} & \text{if } \fv{\PP} \neq \Set{x, y}\text{, } \mathsf{\overline{k}} \in \Set{x, y} \setminus \Set{\mathsf{k}}\text{,}\\
				\hspace{1.5em} \OR \left( \sum_{j \in J} \ssout{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{i}}\seq\sinprlbl{\enodei{\overline{k}}}{\lab_i}{z}\seq\ArbitraryEncoding{\Gamma_j \vdash \PP_j}_{\mathsf{\overline{k}}} \right) & \phantom{if }\text{and } \PP \text{ is typed as internal in } \Gamma\\
				\pa{\enodei{k}}{\left( \sum_{i \in I} \ssinp{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{i}}\seq\soutprlbl{\enodei{\overline{k}}}{\lab_i}{v_i}\seq\ArbitraryEncoding{\Gamma_i \vdash \PP_i}_{\mathsf{\overline{k}}} \right)} & \text{if } \fv{\PP} \neq \Set{x, y}\text{, } \mathsf{\overline{k}} \in \Set{x, y} \setminus \Set{\mathsf{k}}\text{,}\\
				\hspace{1.5em} \OR \left( \sum_{j \in J} \sinprlbl{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{o}}{z}\seq\ArbitraryEncoding{\Gamma_j \vdash \PP_j}_{\mathsf{\overline{k}}} \right) & \phantom{if }\text{and } \PP \text{ is typed as external in } \Gamma
			\end{cases}
		\end{array} $\\
		\hline
	\end{tabular}
	\caption{Keys to Separation and Encodability Results\label{fig:KeysExpressiveness}}
\end{figure*}
}


==> figures/fig-hierarchy-with-theorems.tex <==
\begin{figure*}
	\renewcommand{\arraystretch}{1.2}
	\arraycolsep2pt
	\begin{tabular}{|l|l|c|}
		\hline
		1 &
		$ \begin{array}{l}
			\scbs \blueArrow \bs\\
			\smpst \blueArrow \mpst
		\end{array} $ &
		$ \begin{array}{rcl}
			\ArbitraryEncoding{\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I}} &=& \choice{\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I}\\
			\ArbitraryEncoding{\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J}} &=& \colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J}
		\end{array} $\\
		\hline
		2 &
		$ \begin{array}{l}
			\mcbs \blueArrow \scbs\\
			\dmpst \blueArrow \smpst
		\end{array} $ &
		$ \begin{array}{l}
			\ArbitraryEncoding{\left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I} \right) \OR \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J} \right)}\\
			= \begin{cases}
				\begin{array}{l}
					\left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right) \OR\\
					\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\left( \left(\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{yellow!30}{\ssinp{\q}{\lbl{reset}}}\seq \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right)
				\end{array} & \text{if } I \neq \emptyset \neq J \wedge \p < \q\\
				\left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } I \neq \emptyset \neq J \wedge \p > \q\\
				\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p < \q\\
				\colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p > \q\\
				\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} & \text{if } I = \emptyset \wedge \p < \q\\
				\left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\colorbox{yellow!30}{\ssout{\q}{\lbl{reset}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} & \text{if } I = \emptyset \wedge \p > \q
			\end{cases}
		\end{array} $\\
		\hline
		3 &
		$ \begin{array}{l}
			\mcbs \blueArrow \bs\\
			\dmpst \blueArrow \mpst
		\end{array} $ &
		$ \begin{array}{l}
			\ArbitraryEncoding{\left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I} \right) \OR \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J} \right)}\\
			= \begin{cases}
				\begin{array}{l}
					\left( \choice{\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right) \OR\\
					\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\left( \left(\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{yellow!30}{\ssinp{\q}{\lbl{reset}}}\seq \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right)
				\end{array} & \text{if } I \neq \emptyset \neq J \wedge \p < \q\\
				\colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\left( \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} \right) & \text{if } I \neq \emptyset \neq J \wedge \p > \q\\
				\choice{\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p < \q\\
				\colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\ArbitraryEncoding{\PP_i}}{i \in I} & \text{if } J = \emptyset \wedge \p > \q\\
				\colorbox{green!20}{\ssinp{\q}{\lbl{enc_o}}}\seq\colorbox{red!10}{\ssout{\q}{\lbl{enc_i}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} & \text{if } I = \emptyset \wedge \p < \q\\
				\colorbox{green!20}{\ssout{\q}{\lbl{enc_o}}}\seq\left( \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) \OR \colorbox{red!10}{\ssinp{\q}{\lbl{enc_i}}}\seq\colorbox{yellow!30}{\ssout{\q}{\lbl{reset}}}\seq\choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\ArbitraryEncoding{\PP_j}}{j \in J} \right) & \text{if } I = \emptyset \wedge \p > \q
			\end{cases}
		\end{array} $\\
		\hline
		\multirow{2}{*}{4} &
		\multirow{2}{*}{\mpst \redArrow \mcbs} &
		three distributable steps in\\
		&& $ M_{\mpst} = \pa{\role{a}}{\left( \ssout{\role{b}}{l}\seq\success \OR \ssout{\role{b}}{l}\seq\inact \right)} \Par \pa{\role{b}}{\ssinp{\role{a}}{l}\seq\inact} \Par \pa{\role{c}}{\left( \ssout{\role{d}}{l}\seq\success \OR \ssout{\role{d}}{l}\seq\inact \right)} \Par \pa{\role{d}}{\ssinp{\role{c}}{l}\seq\inact} \Par \pa{\role{e}}{\left( \ssout{\role{f}}{l}\seq\success \OR \ssout{\role{f}}{l}\seq\inact \right)} \Par \pa{\role{f}}{\ssinp{\role{e}}{l}\seq\inact} $\\
		\hline
		\multirow{2}{*}{5} &
		\scmpst \redArrow &
		the synchronisation pattern \patternM in\\
		& Bottom Layer &
		$ \PM_{\scmpst} = \pa{\enodei{a}} \left( \ssout{\enodei{b}}{l}. \ssout{\enodei{d}}{l}. \inact \OR \ssout{\enodei{d}}{l'}. \inact \right) \Par \pa{\enodei{b}} \left( \ssinp{\enodei{a}}{l}. \inact \OR \ssinp{\enodei{c}}{l}. \inact \right) \Par \pa{\enodei{c}} \left( \ssout{\enodei{b}}{l}. \inact \OR \ssout{\enodei{d}}{l}. \inact \right) \Par \pa{\enodei{d}} \left( \ssinp{\enodei{c}}{l}. \ssinp{\enodei{a}}{l}. \success \OR \ssinp{\enodei{a}}{l'}. \inact \right) $\\
		\hline
		\multirow{2}{*}{6} &
		\cnv \redArrow &
		the synchronisation pattern \patternM in\\
		& Bottom Layer &
		$ \PM_{\cnv} = \ResCMV{x}{y}{\left( \OutCMV{x}{\true}{\inactCMV} \Par \InpCMV{\linCMV}{y}{z}{\ConditionalCMV{z}{\inact}{\inactCMV}} \Par \OutCMV{x}{\false}{\inactCMV} \Par \InpCMV{\linCMV}{y}{z}{\ConditionalCMV{z}{\inactCMV}{\success}} \right)} $\\
		\hline
		\multirow{2}{*}{7} &
		\cnvms \redArrow &
		the synchronisation pattern \patternM in\\
		& Bottom Layer &
		$ \PM_{\text{\cnvms}} = \ResCMVmix{x}{y}{\left( \ChoiceCMVmix{\linCMV}{x}{\OutCMVmix{l}{\true}{\inactCMVmix}} \Par \ChoiceCMVmix{\linCMV}{y}{\InpCMVmix{l}{z}{\ConditionalCMVmix{z}{\inact}{\inactCMVmix}}} \Par \ChoiceCMVmix{\linCMV}{x}{\OutCMVmix{l}{\false}{\inactCMVmix}} \Par \ChoiceCMVmix{\linCMV}{y}{\InpCMVmix{l}{z}{\ConditionalCMVmix{z}{\inactCMVmix}{\success}}} \right)} $\\
		\hline
		\multirow{4}{*}{8} &
		& the synchronisation pattern \patternStar in\\
		& \msmpst \redArrow &
		$ \PS_{\msmpst} = M_{\enodei{a}} \Par M_{\enodei{b}} \Par M_{\enodei{c}} \Par M_{\enodei{d}} \Par M_{\enodei{e}} \Par M_{\enodei{gc}} \hspace{2em} M_{\enodei{a}} = \pa{\enodei{a}} \left( \ssout{\enodei{e}}{l}. \inact \OR \ssinp{\enodei{b}}{l}. P_{\enodei{a}} \OR \ssinp{\enodei{gc}}{\delete}. \inact \right) $\\
		& Lower Layers &
		$ M_{\enodei{gc}} = \choice{\ssout{\enodei{i}}{\delete} \seq \inact}{\enodei{i} \in \set{\enodei{a}, \enodei{b}, \enodei{c}, \enodei{d},\enodei{e}}} \hspace{2em} \sigma = \left[ \enodei{a} \mapsto \enodei{b}, \enodei{b} \mapsto \enodei{c}, \enodei{c} \mapsto \enodei{d}, \enodei{d} \mapsto \enodei{e}, \enodei{e} \mapsto \enodei{a} \right] $\\
		&& $ M_{\enodei{b}} = M_{\enodei{a}}\sigma \quad M_{\enodei{c}} = M_{\enodei{b}}\sigma \quad M_{\enodei{d}} = M_{\enodei{c}}\sigma \quad M_{\enodei{e}} = M_{\enodei{d}}\sigma \hspace{2em} P_{\enodei{a}}, \ldots, P_{\enodei{e}} \in \left\{ \success, \inact \right\} $\\[1mm]
		\hline
		9 &
		\mcmpst \blueArrow \msmpst &
		$ \begin{array}{l}
\ArbitraryEncoding{\sum_{\q} \left( \left( \choice{\soutprlbl{\q}{\lab_i}{v_i}\seq\PP_i}{i \in I} \right) \OR \left( \choice{\sinprlbl{\q}{\lab_j}{x_j}\seq\PP_j}{j \in J} \right) \right)} %\\
			= \sum_{\q}
			\begin{cases}
				\text{case distinction of \mcbs \blueArrow \scbs}
			\end{cases}
		\end{array} $\\[1mm]
		\hline
		10 &
		\mcbs \redArrow \lcnvms &
		$ M_{\mcbs} = \pa{\p}{\left( \ssout{\q}{l_1}\seq\inact \OR \colorbox{orange!20}{\ensuremath{\ssinp{\q}{l_2}\seq\success}} \right)} \Par \pa{\q}{\left( \ssinp{\p}{l_1}\seq\inact \OR \colorbox{orange!20}{\ensuremath{\ssinp{\p}{l_3}\seq\success}} \right)} $\\
		\hline
		11 &
		\lcnvms \blueArrow \mcbs &
		$ \begin{array}{l}
\, 			\ArbitraryEncoding{\Gamma \vdash \ResCMVmix{x}{y}{\PP}} = \ArbitraryEncoding{\Gamma' \vdash \PP}_{x, y}\\
			\ArbitraryEncoding{\Gamma \vdash \ChoiceCMVmix{\linCMVmix}{\mathsf{k}}{\left( \PP = \left( \sum_{i \in I} \OutCMVmix{\lab_i}{v_i}{\PP_i} \right) \OR \left( \sum_{j \in J} \InpCMVmix{\lab_j}{z_j}{\PP_j} \right) \right)}}_{x, y}\\
			= \begin{cases}
				\pa{\enodei{k}}{\inact} & \text{if } \fv{\PP} = \Set{x, y} \cup \Set{\mathsf{k}}\\\
				\pa{\enodei{k}}{\left( \sum_{i \in I} \soutprlbl{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{o}}{v_i}\seq\ArbitraryEncoding{\Gamma_i \vdash \PP_i}_{\mathsf{\overline{k}}} \right)} & \text{if } \fv{\PP} \neq \Set{x, y}\text{, } \mathsf{\overline{k}} \in \Set{x, y} \setminus \Set{\mathsf{k}}\text{,}\\
				\hspace{1.5em} \OR \left( \sum_{j \in J} \ssout{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{i}}\seq\sinprlbl{\enodei{\overline{k}}}{\lab_i}{z}\seq\ArbitraryEncoding{\Gamma_j \vdash \PP_j}_{\mathsf{\overline{k}}} \right) & \phantom{if }\text{and } \PP \text{ is typed as internal in } \Gamma\\
				\pa{\enodei{k}}{\left( \sum_{i \in I} \ssinp{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{i}}\seq\soutprlbl{\enodei{\overline{k}}}{\lab_i}{v_i}\seq\ArbitraryEncoding{\Gamma_i \vdash \PP_i}_{\mathsf{\overline{k}}} \right)} & \text{if } \fv{\PP} \neq \Set{x, y}\text{, } \mathsf{\overline{k}} \in \Set{x, y} \setminus \Set{\mathsf{k}}\text{,}\\
				\hspace{1.5em} \OR \left( \sum_{j \in J} \sinprlbl{\enodei{\overline{k}}}{\lab_i \cdot \colorbox{blue!10}{o}}{z}\seq\ArbitraryEncoding{\Gamma_j \vdash \PP_j}_{\mathsf{\overline{k}}} \right) & \phantom{if }\text{and } \PP \text{ is typed as external in } \Gamma
			\end{cases}
		\end{array} $\\
		\hline
	\end{tabular}
	\caption{Keys to Separation and Encodability Results\label{fig:KeysExpressiveness}}
\end{figure*}


==> figures/old_fig_type_lts.tex <==
\begin{figure}
	\hspace*{-8mm}
	$
		\small
		\begin{array}{c}
\begin{array}{rrrr}
\LOut &\hspace{-5mm} \LInp &\hspace{-5mm} \LChoice &\hspace{-5mm} \LRec\\[-1mm]
			\localise{\p} \toutlbl{\q}{\lab}{\UType} \local
			\by{\actoutlbl{\p}{\q}{\lab}{\UType}}
                        \localise{\p} \local
&%\hspace{-5mm} 			
% \ \ \ \LOut 			\quad 
			\localise{\p} \tinplbl{\q}{\lab}{\UType}
                        \local \by{\actinplbl{\p}{\q}{\lab}{\UType}}
            \localise{\p} \local 
%\ \ \ \LInp
%\\[2mm]
&%\hspace{-5mm}  
			\tree {
				\localise{\p} \locali{j} \by{\lambda} \localise{\p} \locald \ j \in I
			}{
				\localise{\p}{\Tor{i \in I}{\locali{i}}} \by{\lambda} \localise{\p} \locald
			}{}%\LChoice}
%\quad                         
& \hspace{-5mm} 
			\tree{
				\localise{\p} \local \subst{\trec{t}{\local}}{\tvar{t}} \by{\lambda} \localise{\p} \locald
			}{
				\localise{\p} \trec{t}{\local} \by{\lambda} \localise{\p} \locald
			}{}%\LRec}
			\end{array}
\\[7mm]
			\tree {
% With subtyping 
%%				\localise{\p} \locali{1} \by{\actoutlbl{\p}{\q}{\lab}{\UTypei{1}}} \localise{\p} \localid{1}
%				\quad
%				\localise{\q} \locali{2} \by{\actinplbl{\q}{\p}{\lab}{\UTypei{2}}} \localise{\q} \localid{2}
%				\quad \UTypei{1} \subt \UTypei{2}
				\localise{\p} \locali{1} \by{\actoutlbl{\p}{\q}{\lab}{\UTypei{}}} \localise{\p} \localid{1}
				\quad
				\localise{\q} \locali{2} \by{\actinplbl{\q}{\p}{\lab}{\UTypei{}}} \localise{\q} \localid{2}
			}{
				\LL, \localise{\p} \locali{1}, \localise{\q} \locali{2}
				\by{\actlbl{\p}{\q}{\lab}{\UTypei{}}}
				\LL, \localise{\p} \localid{1}, \localise{\q} \localid{2}
			}{\RPass}
\\[2mm]                        
			%    \qquad
			%	\tree {
			%	  \begin{array}{l}
			%	  		\forall, i \in \set{1, 2},
			%			\localise{\p} \locali{i} \by{\actout{\p}{\q}{\gr_i}} \localise{\p} \localid{i}
			%			%\ \ 
			%			%\localise{\q} \local_2 \by{\actinp{\q}{\p}{\gr_2}} \localise{\q} \local_2'
			%			\quad 
			%			\gr_1 \not= \gr_2
			%		\end{array}
			%	}{
			%		\LL, \localise{\p} \locali{1}, \localise{\q} \locali{2}
			%		\by{\acterr}
			%		\LL, \localise{\p} \localid{1}, \localise{\q} \localid{2}
			%	}{\EGround}
			%                \qquad
		\end{array}
$\\[-3mm]
%\Description{Semantics for global types, roles, and sets of roles}
\caption{Labelled transition systems of local type and local contexts \label{fig:type_semantics}}
\vspace*{-5mm}
\end{figure}


==> full_ack.tex <==
\paragraph*{\bf Acknowledgements. } 
Work partially supported by: EPSRC EP/T006544/2, EP/K011715/1,
EP/K034413/1, EP/L00058X/1, EP/N027833/2,  EP/N028201/1, EP/T014709/2,
EP/V000462/1, EP/X015955/1, NCSS/EPSRC VeTSS, and Horizon EU
TaRDIS 101093006. We thank Dimitrios Kouzapas for his collaboration
on an early version of a related topic. 



==> intro.tex <==
\section{Introduction}
\label{sec:intro}
\emph{Mixed choice}, which allows non-deterministic
choice between enabled inputs or outputs, 
has been used to represent mutual exclusion such as 
semaphores and concurrent scheduling algorithms in communicating 
systems \cite{CCS}. 
Mixed choice offers the ability to rule out
alternative options, i.e., discard inputs by selecting an output in
the same choice, and vice versa. 
In concurrent and message-passing programming 
languages, there has been interest 
in including and efficiently implementing mixed
choice, as exemplified by 
Concurrent ML
\cite{CML,RRY09}, and
more recently by Go \cite{golang} (where choice is
synchronous by default). 
In Esterel \cite{BERRY199287} 
and Facile \cite{facile96},    
 mixed choice is used 
as a key construct 
to lump all 
IO-synchronisations among parallel processes
as a single choice.

This paper shows that 
an introduction of mixed choice 
in the behavioural type 
theory based on protocols, \emph{multiparty session types}
\cite{HYC08} (\mpst), 
not only offers more safe and deadlock-free processes, 
but also gains \emph{expressiveness} \cite{DBLP:journals/iandc/Gorla10, DBLP:journals/corr/PetersG15},  which was not the case in 
binary (two-party) mixed sessions by \citet{CASAL202223}. 

\myparagraph{Two Party Mixed Choice Sessions.\ }
Session types \cite{THK,honda.vasconcelos.kubo:language-primitives,yoshida.vasconcelos:language-primitives} 
govern communication behaviours 
of concurrent programs, ensuring
\emph{type error freedom} and  
\emph{communication safety} 
(no mismatch between sent and expected data types).
The shape of session types originated in Linear Logic 
\cite{HondaK:typdyi,GirardJY:linlog},
where choices are \emph{separated} (not mixed) and 
\emph{binary} (between two participants). Such choices are 
either a sum of inputs (\emph{external} choice) or 
of outputs (\emph{internal} choice). 

Using session process notation, we can write
\emph{external choice} and 
\emph{internal choice} processes as:\\[1mm] 
\centerline{$P_{\&} \ = \
\sinprlbl{s}{\lab_1}{x_1}.P_1 +
\sinprlbl{s}{\lab_2}{x_2}.P_2$}\\[1mm]
\centerline{
$Q_{\oplus} = \text{if} \ v \ \text{then} \  \soutprlbl{s}{\lab_1}{v_1}.Q_1
\ \text{else} \ 
\soutprlbl{s}{\lab_2}{v_2}.Q_2
$}\\[1mm] 
Here 
$\outmark$ denotes output, 
$\inpmark$ denotes input, and 
$\ell$ is a \emph{label}
used for matching. 
The input process $\sinprlbl{s}{\lab_1}{x_1}.P_1$ 
indicates that the recipient at channel $s$ expects to
receive a value with label $\ell_1$, after which it will continue with behaviour 
$P_1\subst{v_1}{x_1}$.
The output 
$\soutprlbl{s}{\lab_1}{v_1}.Q_1$ 
selects 
label $\ell_1$, sending value $v_1$ and continues as $Q_1$.

A natural next step is the extension of separate 
binary choice to  
\emph{mixed choice} 
(a mixture of synchronous input and outputs in a single choice), 
making it \emph{non-deterministic}, e.g.,
a process waits for 
an input on label $\ell_1$, or can
\emph{non-deterministically} select to output $\ell_2$: \\[1mm]
\centerline{
$P_{+} \ = \
\sinprlbl{s}{\lab_1}{x_1}.P_1 +
\soutprlbl{s}{\lab_2}{v_2}.P_2
\quad 
Q_{+} = \soutprlbl{s}{\lab_1}{v_1}.Q_1 +
\sinprlbl{s}{\lab_2}{x_2}.Q_2$
}\\[1mm]
where 
a parallel composition of $P_{+}$ and $Q_{+}$ synchronises (reduces) either to 
$P_1\subst{v_1}{x_1} \Par Q_1$ or 
$P_2 \Par Q_2\subst{v_2}{x_2}$. 
\NY{This mixed choice behaviour follows the standard 
CCS semantics \cite{CCS}: an output action always chooses a receive action at a choice in another process, and they are synchronised together.} 
Recently, 
\citet{CASAL202223} 
studied this extension (denoted by \cnvms), and proved its type safety. 

\myparagraph{Expressiveness. }
A standard method to compare the abstract \emph{expressive power} of process calculi is to analyse the existence of encodings, \ie translations from one calculus into another.
To rule out trivial or meaningless encodings, they are augmented with a set of quality criteria.
An \emph{encodability} result, \ie an encoding from a \emph{source calculus} into a \emph{target calculus} that satisfies relevant criteria, shows that the target can mimic or \emph{emulate} the behaviours of the source---the target is at least as expressive as the source.
Conversely, a \emph{separation} result, \ie the proof that there is no encoding satisfying the considered criteria, shows that some behaviours of the source cannot be emulated by the target.
The combination of encodability and separation results can build hierarchies of the analysed calculi, if these results are based on the same set of criteria. 
Encodings become stronger by using a stronger criteria, whereas separations become stronger by using weaker criteria.
Sets of criteria that are well suited for encodability and separation were discussed \eg in \cite{Palamidessi03, DBLP:journals/entcs/Parrow08, gorla09, DBLP:journals/iandc/Gorla10, DBLP:journals/tcs/FuL10, DBLP:journals/corr/abs-1208-2750, peters12, PetersN12, DBLP:conf/esop/PetersNG13, DBLP:journals/corr/PetersG15, fu16, glabbeek18, peters19}.
By following in particular \cite{DBLP:journals/iandc/Gorla10, DBLP:conf/esop/PetersNG13}, we consider the criteria \emph{compositionality} (the encoding is a function on the operators of the source), \emph{name invariance} (the encoding treats all names of the source in the same way), sound and complete \emph{operational correspondence} (the encoding preserves and reflects the behaviours of the source), \emph{divergence reflection} (the target diverges only if the source diverges), \emph{success-sensitiveness} (reachability of success is preserved and reflected), and \emph{distributability preservation} (the target has the same degree of distribution as the source).
Encodings that satisfy these criteria are denoted as \emph{good} encodings.

Unfortunately, \citet{PY2022} have shown that 
mixed sessions (\cnvms) proposed by \citet{CASAL202223} do \emph{not} add  
any expressive power 
to the binary session calculus (denoted by \cnv)  \cite{VASCONCELOS201252}  
which has the standard branching and selection constructs (i.e., separate 
choices). 
This is perhaps surprising as it is against a landmark result on expressiveness  by \citet{Palamidessi03}---the $ \pi $-calculus \cite{short:MilnerR:calmp1} with mixed choice is strictly more expressive than the $ \pi $-calculus without choice.
%On the other hand, \citet{CASAL202223} have provided an encoding from \cnvms into \cnv, a fundamental binary sessions with selection and  branching (separated choice) \cite{VASCONCELOS201252}, and proved most of the above mentioned encoding criteria except for the soundness of operational correspondence, which was left open. 
%This problem was solved in \cite{PY2022}.
%Further \citet{CASAL202223} provided a good encoding from \cnv into \cnvms.
%This concludes that \cnvms and \cnv have the same expressive power, \ie mixed choice adds no more expressiveness in binary sessions in \cite{VASCONCELOS201252}.
An open question is under which circumstances, mixed choice in session types
is strictly more expressive. 

\myparagraph{Expressiveness Hierarchy with Binary Mixed Sessions.\ }
To explain the above open problem more precisely, we first 
present a hierarchy of $ \pi $-like calculi from \cite{PY2022}
in Figure~\ref{fig:hierarchyPi}.

\input{figures/fig_pi_hierarchy}

\noindent
\begin{minipage}{\columnwidth}
	\begin{wrapfigure}{R}{0.25\columnwidth}
		\hspace*{-2em}
		\scalebox{0.65}{
		\tikzstyle{place}=[circle,draw=black,thick,minimum size=5mm]
		\tikzstyle{transition}=[rectangle,draw=black,thick,minimum size=5mm]
		\begin{tikzpicture}
			% fully reachable pure M in Petri Nets
			\node[place,tokens=1]	(p) at (0.75, 1.5) {};
			\node[place,tokens=1]	(q) at (2.25, 1.5) {};
			\node[transition]		(a) at (0, 0) {$ a $};
			\node[transition]		(b) at (1.5, 0) {$ b $};
			\node[transition]		(c) at (3, 0) {$ c $};
			\draw[-latex] (p) -- (a);
			\draw[-latex] (p) -- (b);
			\draw[-latex] (q) -- (b);
			\draw[-latex] (q) -- (c);
		\end{tikzpicture}
		}
	\end{wrapfigure}
\smallskip

The hierarchy orders calculi along their ability to express the \emph{synchronisation patterns} \patternM and \patternStar.
An \patternM (see \cite{Glabbeek2008, glabbeekGoltzSchicke12}), as visualised on the right, describes a Petri net that consists of two parallel transitions ($ a $ and $ c $) and one transition ($ b $) that is in conflict with both of the former.
	In other words, it describes a situation where either two parts of the net can proceed independently or they synchronise to perform a single transition together.

\smallskip

\end{minipage}

As stated by Glabbeek et al. \cite{Glabbeek2008, glabbeekGoltzSchicke12}, a Petri net specification can be implemented in an asynchronous, fully distributed setting iff it does not contain a fully reachable pure \patternM.
They also present a description of a fully reachable pure \patternM as conditions on a state in a step transition system, which allows us to directly use this pattern to reason about process calculi 
%The \patternM pattern is also applicable to examine the expressiveness 
%in process calculi 
%, \ie also allows to separate asynchronous from not purely asynchronous process calculi as shown in 
as shown in \cite{petersSchickeNestmann11, peters12, DBLP:conf/esop/PetersNG13}. 

\noindent
\begin{minipage}{\columnwidth}
	\begin{wrapfigure}{R}{0.25\columnwidth}
		\vspace{-1em}
		\hspace{-2em}
		\scalebox{0.6}{
		\tikzstyle{place}=[circle,draw=black,thick,minimum size=5mm]
		\tikzstyle{transition}=[rectangle,draw=black,thick,minimum size=5mm]
		\begin{tikzpicture}
			\foreach \x/\xtext in {1/e,2/d,3/c,4/b,5/a}
	        {
	            \path (360*\x/5+125:0.8) node[transition] (\xtext) {$\xtext$};
	            \path (360*\x/5-55:1.75) node[place,tokens=1] (p\x) {};
	        }
	        \draw[-latex] (p2) -- (a);
	        \draw[-latex] (p2) -- (b);
	        \draw[-latex] (p1) -- (b);
	        \draw[-latex] (p1) -- (c);
	        \draw[-latex] (p5) -- (c);
	        \draw[-latex] (p5) -- (d);
	        \draw[-latex] (p4) -- (d);
	        \draw[-latex] (p4) -- (e);
	        \draw[-latex] (p3) -- (e);
	        \draw[-latex] (p3) -- (a);
		\end{tikzpicture}
		}
		\vspace{-1em}
	\end{wrapfigure}

\smallskip

Further, Peters et al.~\cite{peters12, DBLP:conf/esop/PetersNG13} introduce the synchronisation pattern \patternStar, 
which is a chain of conflicting and distributable steps as they occur in an \patternM that build a circle of odd length.
	As visualised on the right, there is \eg one \patternM consisting of the transitions $ a $, $ b $, and $ c $ with their corresponding two places.
	Another \patternM is build by the transitions $ b $, $ c $, and $ d $ with their corresponding two places and so on.

\smallskip
\end{minipage}

The \patternM captures only a small amount of synchronisation, whereas the \patternStar requires considerably more synchronisation in the calculus.
\emph{Asynchronously distributed calculi} that cannot express \patternM nor \patternStar such as the $ \mathsf{Join} $-calculus from \cite{fournet.gonthier:join} are placed in the bottom layer of Figure~\ref{fig:hierarchyPi}.
\emph{Synchronously distributed calculi} that can express \patternStar and thus also \patternM such as the $ \pi $-calculus with mixed choice ($ \pi $) are placed in the top layer.
The middle layer consists of the calculi that can 
express \patternM but not \patternStar. 
%, \ie calculi with some synchronisation features but without the expressive power of synchronous calculi.
The asynchronous $\pi$-calculus without choice \cite{HondaTokoro91,Boudol92} 
($\pi_{\mathsf{a}}$),
the $ \pi $-calculus 
with separate choice \cite{Nestmann00}
($\pi_{\mathsf{s}}$),
and mobile ambients \cite{CardelliL:mobamb} ($ \mathsf{MA} $)
are placed in the middle---unless it is restricted to unique ambient names ($ \mathsf{MA}_{\mathsf{u}} $) \cite{petersNestmannIC20}.
That \cnv and \cnvms are also placed in the middle layer was proven in \cite{PY2022}.
Hence, they are \emph{strictly less expressive} than $ \pi $.
This completes Figure~\ref{fig:hierarchyPi}.   
% Related 
%On the other hand, \citet{CASAL202223} have provided an encoding from \cnvms into \cnv, a fundamental binary sessions with selection and 
%branching (separated choice) \cite{VASCONCELOS201252}, and proved 
%most of the above mentioned encoding criteria except 
%for the soundness of operational correspondence, which had left opened. 
%This problem was solved in \cite{PY2022}. 
%Further \citet{CASAL202223} provided 
%a good encoding from \cnv into \cnvms. 
%This concludes that \cnvms and \cnv have the same expressive power, 
%\ie mixed choice adds no more expressiveness in binary sessions  
%in \cite{VASCONCELOS201252}. 
%An open question is under which circumstances, mixed choice in session types
%can increase the expressive power.
%We observe that the key is multiparty sessions with choice 
%in which input and output prefixes interact 
%towards different communication partners. 

\myparagraph{Mixed Choice Multiparty Session Types.}
In the presence of 
mixed choice, 
the extension from two parties to \emph{more than two} parties
gives us strictly more expressive power to session types and is placed in the top layer. 
This is because 
not only inputs and outputs but also 
\emph{destinations of messages} represented by \emph{participants}
can be mixed in one single choice.

Consider three participants
$\role{a}$, $\role{b}$, and $\role{c}$, and  
assume $P_{\role{a}}$, $P_{\role{b}}$ and $P_{\role{c}}$ below:\\[1mm]
\centerline{
$P_{\role{a}} = 
(\tout{\role{b}}{\ell_1}{
 \ntout{\role{c}}{\ell_2}{}})
+
\ntinp{\role{b}}{\ell_1}{}
+
\ntinp{\role{c}}{\ell_2}{}
\quad
P_{\role{b}} = 
\ntinp{\role{a}}{\ell_1}{}
+
(\tout{\role{a}}{\ell_1}{\ntout{\role{c}}{\ell_2}{}})
+
\ntinp{\role{c}}{\ell_2}{}$}\\[1mm]
\centerline{
$P_{\role{c}} = 
\ntinp{\role{a}}{\ell_2}{}
+
\ntinp{\role{b}}{\ell_2}{}
+
(\tout{\role{a}}{\ell_2}{\ntout{\role{b}}{\ell_2}{}})$}\\[1mm]
where we omit the payload and nil processes. In multiparty sessions,
each process who plays role $\p$
is represented as $\pa{\p}{\PP}$. Assuming, e.g.,  
$\ntout{\role{b}}{\ell_1}$ in $P_{\role{a}}$ matches with
$\ntinp{\role{a}}{\ell_1}$ in $P_{\role{b}}$,
their parallel composition 
$(\pa{\role{a}}{\PP_{\role{a}}}
\Par 
\pa{\role{b}}{\PP_{\role{b}}}
\Par 
\pa{\role{c}}{\PP_{\role{c}}})$ 
non-deterministically leads 
to several possible states such as 
$\pa{\role{a}}{\ntout{\role{c}}{\ell_2}{}}
\Par 
\pa{\role{c}}{\PP_{\role{c}}}$ 
or 
$\pa{\role{b}}{\PP_{\role{b}}}
\Par 
\pa{\role{c}}{\ntout{\role{b}}{\ell_2}{}}$.  
We can observe that the choice behaviours of processes are 
\emph{distributed} to and from two distinct participants.
%We introduce a variant of multiparty session types, called \mcmpst, that contains such processes.
%In order to focus on mixed choice within sessions, we consider in \mcmpst only a single session and no session initialisation.

%\myparagraph{Expressiveness heirarchy with binary mixed sessions.\ }
%Figure~\ref{fig:hierarchyPi} presents a hierarchy of $ \pi $-like calculi from \cite{PY2022}.
%
%\input{figures/fig_pi_hierarchy}
%
%\noindent
%\begin{minipage}{\columnwidth}
%	\begin{wrapfigure}{R}{0.25\columnwidth}
%		\hspace*{-1.5em}
%		\scalebox{0.6}{
%		\tikzstyle{place}=[circle,draw=black,thick,minimum size=5mm]
%		\tikzstyle{transition}=[rectangle,draw=black,thick,minimum size=5mm]
%		\begin{tikzpicture}
%			% fully reachable pure M in Petri Nets
%			\node[place,tokens=1]	(p) at (0.75, 1.5) {};
%			\node[place,tokens=1]	(q) at (2.25, 1.5) {};
%			\node[transition]		(a) at (0, 0) {$ a $};
%			\node[transition]		(b) at (1.5, 0) {$ b $};
%			\node[transition]		(c) at (3, 0) {$ c $};
%			\draw[-latex] (p) -- (a);
%			\draw[-latex] (p) -- (b);
%			\draw[-latex] (q) -- (b);
%			\draw[-latex] (q) -- (c);
%		\end{tikzpicture}
%		}
%	\end{wrapfigure}
%
%	\quad The hierarchy orders calculi along their ability to express the \emph{synchronisation patterns} \patternM and \patternStar.
%An \patternM (see \cite{Glabbeek2008, glabbeekGoltzSchicke12}), as visualised on the right, describes a Petri net that consists of two parallel transitions ($ a $ and $ c $) and one transition ($ b $) that is in conflict with both of the former.
%	In other words, it describes a situation where either two parts of the net can proceed independently or they synchronise to perform a single transition together.
%\end{minipage}
%
%As stated in \cite{Glabbeek2008, glabbeekGoltzSchicke12}, a Petri net specification can be implemented in an asynchronous, fully distributed setting iff it does not contain a fully reachable pure \patternM.
%They also present a description of a fully reachable pure \patternM as conditions on a state in a step transition system, which allows us to directly use this pattern to reason about process calculi.
%The \patternM pattern is also applicable in process calculi, \ie also allows to separate asynchronous from not purely asynchronous process calculi as shown in \cite{petersSchickeNestmann11, peters12, DBLP:conf/esop/PetersNG13}. 
%
%\noindent
%\begin{minipage}{\columnwidth}
%	\begin{wrapfigure}{R}{0.25\columnwidth}
%		\vspace{-1em}
%		\hspace{-2em}
%		\scalebox{0.6}{
%		\tikzstyle{place}=[circle,draw=black,thick,minimum size=5mm]
%		\tikzstyle{transition}=[rectangle,draw=black,thick,minimum size=5mm]
%		\begin{tikzpicture}
%			\foreach \x/\xtext in {1/e,2/d,3/c,4/b,5/a}
%	        {
%	            \path (360*\x/5+125:0.8) node[transition] (\xtext) {$\xtext$};
%	            \path (360*\x/5-55:1.75) node[place,tokens=1] (p\x) {};
%	        }
%	        \draw[-latex] (p2) -- (a);
%	        \draw[-latex] (p2) -- (b);
%	        \draw[-latex] (p1) -- (b);
%	        \draw[-latex] (p1) -- (c);
%	        \draw[-latex] (p5) -- (c);
%	        \draw[-latex] (p5) -- (d);
%	        \draw[-latex] (p4) -- (d);
%	        \draw[-latex] (p4) -- (e);
%	        \draw[-latex] (p3) -- (e);
%	        \draw[-latex] (p3) -- (a);
%		\end{tikzpicture}
%		}
%		\vspace{-1em}
%	\end{wrapfigure}
%
%	\quad Further, Peters et al. \cite{peters12,DBLP:conf/esop/PetersNG13} introduce the synchronisation pattern \patternStar, 
%which is a chain of conflicting and distributable steps as they occur in an \patternM that build a circle of odd length.
%	As visualised on the right, there is \eg one \patternM consisting of the transitions $ a $, $ b $, and $ c $ with their corresponding two places.
%	Another \patternM is build by the transitions $ b $, $ c $, and $ d $ with their corresponding two places and so on.
%\end{minipage}
%
%The \patternM captures only a small amount of synchronisation, whereas the \patternStar requires considerably more synchronisation in the calculus.
%Asynchronous calculi---that cannot express \patternM nor \patternStar---such as the $ \mathsf{Join} $-calculus from \cite{fournet.gonthier:join} are placed in the bottom layer of Figure~\ref{fig:hierarchyPi}.
%Synchronous calculi---that can express \patternStar and thus also \patternM---such as the $ \pi $-calculus with mixed choice are placed in the top layer.
%The middle layer is for calculi that can express \patternM but not \patternStar, \ie calculi with some synchronous features but without the expressive power of synchronous calculi.
%As expected, we find in the middle $ \pi_{\mathsf{a}} $ (the asynchronous $ \pi $-calculus without choice introduced independently in \cite{HondaTokoro91} and \cite{Boudol92}) and also $ \pi_{\mathsf{s}} $ (the $ \pi $-calculus with separate choice \cite{Nestmann00}).
%As shown in \cite{petersNestmannIC20}, mobile ambients ($ \mathsf{MA} $) from \cite{CardelliL:mobamb} are also placed in the middle; unless it is restricted to unique ambient names, \ie to the asynchronous $ \mathsf{MA}_{\mathsf{u}} $.
%That \cnv and \cnvms are also in the middle layer, \ie can express \patternM but no \patternStar, was shown in \cite{PY2022} (which completes Figure~\ref{fig:hierarchyPi}).

\myparagraph{Expressiveness in Mixed Choice Multiparty Sessions}
After introducing the typing system of \mcmpst, we study the expressive power introduced by multiparty mixed choice, \ie determine in which layer of Figure~\ref{fig:hierarchyPi}, \mcmpst is situated.
A precise answer to this question was not as simple as expected.
To more clearly understand the causes of an increase in expressiveness, 
we first restrict our attention to a \emph{single multiparty session} 
which has neither shared names, name passings, 
session delegation nor interleaved sessions, and   
consider subcalculi of \mcmpst. 
By limiting the form of the choices and number of participants, \mcmpst includes \emph{9 subcalculi} (including itself).
For example, we can define
\emph{separated choice from/to multiple participants} (\scmpst),  
e.g.,
\\[1mm]  
\centerline{
$P_{\text{\scmpst}}=\tout{\role{a}}{\ell_1}{\tout{\role{b}}{\ell_1}} 
+
\tout{\role{a}}{\ell_2}{\tinp{\role{c}}{\ell_2}}
+ 
\tout{\role{b}}{\ell_3}{\tinp{\role{c}}{\ell_2}}
+
\tout{\role{b}}{\ell_4}{\tinp{\role{a}}{\ell_2}}$
}\\[1mm]
and \emph{directed mixed choice} (\dmpst) 
where choice is mixed but from/to the same participant,  
e.g.,  
\\[1mm]  
\centerline{
$P_{\text{\dmpst}}
=\tout{\role{a}}{\ell_1}{\tout{\role{b}}{\ell_1}} 
+
\ntinp{\role{a}}{\ell_2}{\tinp{\role{c}}{\ell_2}}
+
\tout{\role{a}}{\ell_3}{\tout{\role{b}}{\ell_3}}$
}\\[1mm]
This makes the expressiveness analysis 
very subtle and comprehensive:  
we prove 20 new separation results and 8 
new encodability results among 
9 subcalculi of \mcmpst and 4 variants of \cnvms\ 
\cite{CASAL202223}. 
Our observation is, 
by allowing a \emph{combination of different 
communication patterns in a single choice}, we can cross the boundary of expressiveness. For example, \mcmpst is strictly more expressive than \scmpst 
and can express the pattern \patternStar; and 
\scmpst is strictly more expressive than \dmpst and can 
express pattern \patternM; 
but \dmpst and \mpst have the same expressive power and belong to 
the bottom. 

The highlight is, in spite of the fact that \cnvms enables creating an infinite number of interleaved binary mixed sessions with unrestricted names, \mcmpst 
(a single mixed choice multiparty session) cannot be emulated by \cnvms.
In our results, properties such as \emph{communication safety}  and \emph{deadlock-freedom} \NY{(if a session terminates, then all participants terminate, completing all actions)} ensured by the \mcmpst typing system play the key role to prove the encodability results. 

\myparagraph{Contributions.\ } 
\begin{enumerate*}[=leftmargin]
\item We first introduce the calculus, types and a typing system of 
\emph{mixed choice multiparty sessions} (\mcmpst) which subsume  
the types and typability of the classical synchronous multiparty sessions  
(\mpst). We follow a general \mpst typing system in \cite{less_is_more} which does not require global types. 
We then prove 
\emph{communication safety} and \emph{deadlock-freedom} of typable sessions.
\item \KPCom{We analyse the expressive power of mixed choice in \mcmpst showing that it is strictly more expressive than choice in \mpst.
Therefore we use 8 subcalculi of \mcmpst deliberately chosen to explain the features of choice that raise expressiveness and compare to 4 variants of \cnvms.}
We prove 8 encodability and 20 separation results among the 13 calculi, introducing 8 new \emph{good} encodings. 
\end{enumerate*}
\KPCom{The omitted proofs and more details can be found in \cite{PetersYoshida24tecRep}.} 










==> simple_family.tex <==
\begin{itemize}
\item \mcmpst 

The syntax of this paper 

\item \scmpst 

Separated Choice per participant 

\[
P::=\choice{\soutprlbl{\rolei{p}{i}}{\lab_{ij}}{v_{ij}} \seq \PP_{ij}}{i \in I,j\in J} + 
\choice{\sinprlbl{\rolei{q}{k}}{\lab_{kh}}{v_{kh}} \seq \PP_{kh}}{k \in K,h\in H} \quad \set{\rolei{p}{i}}_{i\in I}\cap \set{\rolei{q}{k}}_{k\in K}=\emptyset
\] 


\item \mpst 

\[
P::=\choice{\soutprlbl{\role{p}{}}{\lab_{i}}{v_{i}} \seq \PP_{ij}}{i \in I} 
\bnfbar 
\choice{\sinprlbl{\role{q}}{\lab_{k}}{v_{k}} \seq \PP_{k}}{k \in K} 
\] 

\item \mcbs a single binary mixed choice session 

(only $\role{p}$ and $\role{q}$ with the syntax of this paper) 
$\role{p}$ is a dual of $\role{q}$. 

\item 

a single binary separate mixed choice session 
(only $\role{p}$ and $\role{q}$) so the syntax of this calculus is the same as 
\bs. 

\item \bs a single binary session (only $\role{p}$ and $\role{q}$) 

\[
P::=\choice{\soutprlbl{\role{p}{}}{\lab_{i}}{v_{i}} \seq \PP_{ij}}{i \in I} 
\bnfbar 
\choice{\sinprlbl{\role{q}}{\lab_{k}}{v_{k}} \seq \PP_{k}}{k \in K} 
\]

\item \cnv Vasco's binary session 
\item \cnvms Vasco's binary mixed sessions 
\item \lcnv Vasco's binary linear sessions 
\item \lcnvms Vasco's binary linear mixed sessions 
\end{itemize}
